A journey towards the most efficient state database for Hyperledger Fabric

The Hyperledger Fabric is well known and the most prominent enterprise-grade permissioned blockchain. The architecture of the Hyperledger Fabric introduces a new architecture paradigm of simulate-order-validate and pluggable architecture, allowing a greater level of customization where one of the critical components is the world state database, which is responsible for capturing the snapshot of the blockchain application state. Hyperledger Fabric manages the state with the key-value database abstraction and peer updates it after transactions have been validated and read from the state during simulation. Therefore, providing good performance during reading and writing impacts the system's overall performance. Currently, Hyperledger Fabric supports two different implementations of the state database. One is LevelDB, the embedded DB based on LSM trees and CouchDB. In this study, we would like to focus on searching and exploring the alternative implementation of a state database and analyze whenever there are better and more scalable options. We evaluated different databases to be plugged into Hyperledger Fabric, such as RocksDB, Boltdb, and BadgerDB. The study describes how to plug new state databases and performance results based on various workloads.

==> live.main.tex <==
undefined

The concept of channels is brought into play by Fabric architecture to facilitate improved data segregation, which protects users' privacy and enables 
sharding, alleviating scalability issues. In addition, the information may be safely traded between consortium members through the channel formed by 
the parties who have organized themselves into a consortium. Channels are a straightforward abstraction of the private blockchain instance's ledger 
management, smart contract administration, and other features. The nodes that participate in the Hyperledger Fabric blockchain network typically 
fulfill one of the following three roles: 

\begin{itemize}
\item The business application code is tasked with coordinating the flow of transaction processing, and it typically 
uses the Fabric SDK to interact with the Hyperledger Fabric.  
\item The endorsing and committing peers are responsible for managing the state, validating transactions, and 
providing attestation of agreement of transaction execution results .
\item Ordering service instituting atomic broadcast abstraction to carry out consensus protocol, 
which is used to group client transactions into blocks and guarantee total order between all transactions.
\end{itemize} 

undefined
